Core-collapse supernovae in dense environments -- particle acceleration and non-thermal emission

Supernova remnants are known to accelerate cosmic-rays from the detection of non-thermal emission in radio waves, X-rays, and gamma-rays. However, the ability to accelerate cosmic-rays up to PeV energies has yet to be demonstrated. The presence of cut-offs in the gamma-ray spectra of several young SNRs led to the idea that PeV energies might only be achieved during the first years of a remnant's evolution. We use our time-dependent acceleration-code RATPaC to study the acceleration of cosmic-rays in supernovae expanding into dense environments around massive stars. We performed spherically symmetric 1-D simulations in which we simultaneously solve the transport equations for cosmic-rays, magnetic turbulence, and the hydrodynamical flow of the thermal plasma in the test-particle limit. We investigated typical CSM parameters expected around RSG and LBV stars for freely expanding winds and accounted for the strong gamma-gamma-absorption in the first days after explosion. The maximum achievable particle energy is limited to below 600TeV even for largest considered values of the magnetic field and mass-loss rates. The maximum energy is not expected to surpass 200TeV and 70TeV for LBVs and RSGs that experience moderate mass-loss prior to the explosion. We find gamma-ray peak-luminosities consistent with current upper limits and evaluated that current-generation instruments are able to detect the gamma-rays from Type-IIP explosions at distances up to 60kpc and Type-IIn explosions up to 1.0Mpc. We also find a good agreement between the thermal X-ray and radio synchrotron emission predicted by our models with a range of observations.

==> defs.tex <==
%
% JOURNALS
%
\providecommand{\nat}{Nature}  
\providecommand{\aanda}{A\&A}  %{\textit{Astronomy \& Astrophysics}}
\providecommand{\aaps}{A\&AS}  %{\textit{Astronomy \&
                           % Astrophysics Supplement series}}
\providecommand{\aap}{A\&A}  %{\textit{Astronomy \& Astrophysics}}
\providecommand{\aapr}{A\&A Rev.}  %{\textit{Astronomy \& Astrophysics}}
\providecommand{\aj}{AJ}      %{\textit{Astronomical Journal}}
\providecommand{\apj}{ApJ}      %{\textit{Astrophysical Journal}}
\providecommand{\apjl}{ApJL}   %{\textit{Astrophysical Journal Letters}}
\providecommand{\apjs}{ApJS}   %{\textit{Astrophysical Journal Supplement}}
\providecommand{\mnras}{MNRAS} %{\textit{Monthly Notices of the R.A.S.}}
\providecommand{\memras}{Mem.~RAS} %{\textit{Mem.~of the R.A.S.}}
\providecommand{\newa}{NewA}   %{\textit{New Astronomy}}
\providecommand{\na}{NewA}
\providecommand{\jcp}{JCP}     %{\textit{Journal of Computational Physics}}
\providecommand{\rmxaa}{RMxAA} %{\textit{Revista Mexicana de Astronom\'ia y Astrof\'isica}}
\providecommand{\pasj}{PASJ}   %{\textit{Publications of the Astronomical Society of Japan}}
\providecommand{\pasp}{PASP}   %{\textit{Publications of the Astronomical Society of Pacific}}
\providecommand{\apss}{AP\&SS} %{\textit{Astrophsycis \& Space Sciences}}
\providecommand{\araa}{ARA\&A} %{\textit{Annual Reviews of Astronomy \& Astrophysics}
\providecommand{\bain}{Bull.~Astron.~Inst.~Netherlands} % {\textit{Bulletin Astronomical Institute of the Netherlands}}
\providecommand{\physrep}{Physics Reports}
\providecommand{\ssr}{Space Science Reviews}
\providecommand{\pre}{Physical Review E}
\providecommand{\jgr}{Journal of Geophysics Research}
